Learning in Auctions: Regret is Hard, Envy is Easy

A line of recent work provides welfare guarantees of simple combinatorial auction formats, such as selling m items via simultaneous second price auctions (SiSPAs) (Christodoulou et al. 2008, Bhawalkar and Roughgarden 2011, Feldman et al. 2013). These guarantees hold even when the auctions are repeatedly executed and players use no-regret learning algorithms. Unfortunately, off-the-shelf no-regret algorithms for these auctions are computationally inefficient as the number of actions is exponential. We show that this obstacle is insurmountable: there are no polynomial-time no-regret algorithms for SiSPAs, unless RP$\supseteq$ NP, even when the bidders are unit-demand. Our lower bound raises the question of how good outcomes polynomially-bounded bidders may discover in such auctions. To answer this question, we propose a novel concept of learning in auctions, termed "no-envy learning." This notion is founded upon Walrasian equilibrium, and we show that it is both efficiently implementable and results in approximately optimal welfare, even when the bidders have fractionally subadditive (XOS) valuations (assuming demand oracles) or coverage valuations (without demand oracles). No-envy learning outcomes are a relaxation of no-regret outcomes, which maintain their approximate welfare optimality while endowing them with computational tractability. Our results extend to other auction formats that have been studied in the literature via the smoothness paradigm. Our results for XOS valuations are enabled by a novel Follow-The-Perturbed-Leader algorithm for settings where the number of experts is infinite, and the payoff function of the learner is non-linear. This algorithm has applications outside of auction settings, such as in security games. Our result for coverage valuations is based on a novel use of convex rounding schemes and a reduction to online convex optimization.

==> contextual-bandits.tex <==
We will apply the results of Section \ref{sec:low-dim} to the adversarial, albeit full information version of the contextual bandit problem \cite{Li2010}, with a finite number of possible contexts $d$ and $N$ alternative actions. A major open question in the contextual bandit literature is whether there exist oracle based algorithms for the adversarial setting. Such algorithms are only known in the stochastic i.i.d. setting (see e.g. \cite{Agarwal2014}. We give the first, oracle-based algorithm for this problem in the adversarial setting, albeit in the complete information setting.

We consider the following setting: at each iteration the adversary picks a context $c^t\in \C$ and a reward vector $r^t\in \R^N$ for each of a set of alternatives $N$ and we denote with $\theta^t=(c^t,r^t)$. We assume $|\C|=d$, i.e. there are $d$ possible contexts. On each day, the player picks a policy $\pi$ which map a context $x$ to an alternative in $[N]$. We denote with $\Pi\subseteq (\C\rightarrow [N])$ the subset of policies which we consider. Thus the set of actions in the online learning formulation is $\Pi\subseteq \C^N$. The utility from an action $\pi$ on each day is given by: $u(\pi,\theta^t)=r_{\pi(x^t)}^t$. Even though our setting is stated as if the contexts are finite, our results extend even if the contexts are infinite, but the policy set that we consider, first classifies each context in one among $d$ possible classes and then uses only the class index to determine the chosen action.

We first show that this setting admits low dimensional sufficient statistics. Basically, all we need to keep track, in order to solve the offline optimization problem for a sequence of parameters $\theta^{1:T}$ is the vector $R_{c,j}^T=\sum_{t\in [T]: c^t=c} r_j^t$ which for each context $c\in C$ and for each action $j\in [N]$, it keeps track of the cumulative utility of alternative $j\in [N]$, on the subset of time-steps when context $x$ appeared. The reason is that for any fixed policy $\pi$:
\begin{align}
\sum_{t=1}^T u(\pi,\theta^t) = \sum_{c\in \C}\sum_{t\in [T]: c^t=c} r_{\pi(c)}^t = \sum_{c\in \C}\sum_{j\in [N]}R_{c,j}^T\cdot 1\{\pi(c)=j\}
\end{align}
Thus the mapping $\phi(\theta^{1:T})$ simply outputs the $d\cdot N$ dimensional vector where coordinate $(c,j)$ contains $R_{c,j}^T$. 

We now argue that this mapping satisfies all properties that we want: 
\begin{enumerate}
\item First it is linear: i.e. $\phi(\{x\}\cup\{y\})=\phi(\{x\})+\phi(\{y\})$.
\item For any sequence $\{x\}$ and parameter $\theta=(c,r)$: 
\begin{equation}\label{eqn:bounded-stat-change}
\|\phi(\{x\}\cup \theta) -\phi(\{x\})\|_1\leq \|r\|_{1}
\end{equation}
Thus if a sequence satisfies, $r_j^t\in [0,H]$, then $\|r\|_1 \leq N\cdot H$.
\end{enumerate}

Last we claim that there is an easy way to induce exponential perturbations in the sufficient statistics space. We add one sample for each context $c\in \C$, in the sequence $\{x\}$. Thus the sequence has fixed length $d$ and the sample $x_c=(c,r_c)$ associated with context $c$, has its reward vector $r_c$, drawn from an coordinate-wise independent symmetric exponential distribution with parameter $\epsilon$.

Thus instantiating Theorem \ref{thm:statistic-regret}, to the above setting we get the following theorem:
\begin{theorem}\label{thm:contextual-regret}
Suppose that we are given an oracle for the offline best-fixed policy problem then algorithm \ref{defn:lazy-ftpl} with an exponentially inducing sample perturbation with parameter $\epsilon = \frac{\sqrt{d\cdot 2 \cdot (\log(N)+1)}}{H\cdot \sqrt{N\cdot T}}$, runs each step in time $O(N)$ and makes one oracle access. Moreover, its regret against any obliviously and adversarially chosen sequence of contexts and rewards $\theta^{1:T}= (c^{1:T},r^{1:T})$ such that $r_j^t\in [0,H]$,  is upper bounded by:
\begin{equation}
\sup_{\pi^*\in \C^N}\E_{\{x\}}\left[\sum_{t=1}^T \left( u(\pi^*,\theta^t) - u(\pi^t,\theta^t)\right)\right] \leq O\left(H\cdot \sqrt{d \cdot N\cdot  \log(N)\cdot T}\right)
\end{equation}
Hence, the regret of Algorithm~\ref{defn:ftpl} against adaptive adversaries is bounded by the same amount. 
\end{theorem}

==> extensions.tex <==


The no-envy learning concept is applicable to general mechanism design settings. By the \emph{taxation principle}, from the perspective of a single bidder and for any bids of the other bidders, any mechanism can be viewed as menu, containing allocation-price pairs. In a learning context, the menu that a bidder faces is changing at every round as a function of the other bids. We can thus define the no-envy guarantee as requiring that the average utility obtained by the bidder in $T$ rounds is at least as high as his value for any allocation less the average price of that allocation across the $T$ rounds. We believe that it is an interesting and fruitful research direction to design no-envy learning algorithms for mechanism design settings beyond the SiSPAS considered in this paper. 


%  We can define "thresholds" for each allocation $x$ as the minimum amount you could have paid to win allocation $x$. Then define no-envy learning that in-retrospect an algorithm achieves approximate no-envy if the average utility is at least $\lambda\cdot v(x)-\mu\cdot\theta(x)$ for any allocation $x$. Then we can show that for many mechanisms that have been studied we can achieve no-envy in polynomial time assuming that the valuation $v(\cdot)$ admits an $\alpha$-approximate convex rounding scheme. We might be able to capture simultaneous multi-unit auctions these way, where e.g. each auction is a uniform price $k$-unit auction. Or we could also capture simultaneous greedy combinatorial auctions or simultaneous position auctions.


==> intro2.tex <==
Suppose you were %that your boss 
assigned %you 
the task of procuring items for a company. There are $m$ items that you may procure, and the company's value for each bundle $S \subseteq [m]$ is specified by a valuation $v: 2^{[m]} \longrightarrow \mathbb{R}$. In fact, suppose that you need to do a fresh procurement every day for $T$ days. Making your task challenging is the fact that, every day, each of the $m$ items is sold separately through a second price auction, and these auctions are run in parallel. So, every day, you are called to place a bid in each single-item auction, and cannot express more complex preferences over bundles of items. Moreover, you have no information about who else may be participating in the various auctions or what their valuations might be, so you cannot predict the prices at which different items will end up selling each day.

Given your lack of information about the competition and your inability to express complex preferences, a natural guarantee you may want to achieve is {\em no-regret}: that your cumulative utility over $T$ procurements is within an additive $o(T)$ of the cumulative utility that you would have achieved in hindsight from the best vector of bids $b_1,\ldots,b_m$, if you were to place the same bid $b_j$ in the second-price auction for item $j$ across all $T$ periods. 

Besides being motivated from an online learning point of view, a growing volume of recent papers has shown that no-regret learning in auction environments also achieves surprising welfare guarantees~\cite{Bikhchandani1999,Christodoulou2008,Bhawalkar2011,Hassidim2011,Syrgkanis2013,Feldman2013}. For example, when bidders whose valuations are subadditive\footnote{A {\em subadditive} valuation $v$ is one satisfying $v(S \cup T) \le v(S)+v(T),$ for all $S, T \subseteq [m]$.} use no-regret learning to choose their bids in repeated simultaneous second-price auctions (SiSPAs), the average welfare converges to a quarter of that achieved by the optimal allocation~\cite{Feldman2013,Duetting2013}. Similar guarantees hold for %SiSPAs or 
other types of compositions of simple auctions~\cite{Syrgkanis2013}. This guarantee is astounding, given the impossibility results for dominant strategy incentive compatible mechanisms, which hold even when the bidders have submodular valuations~\cite{Dobzinski2011,Dughmi2015}.\footnote{A {\em submodular} valuation $v$ is one satisfying $v(S\cup T) + v(S \cap T) \le v(S)+v(T)$, for all $S, T \subseteq [m]$.} 

The robustness of no-regret learning with respect to players' (lack of) information and its strong welfare guarantees motivates us to study its computational complexity. We show that in one of the most basic settings where no-regret learning is non-trivial, it cannot be implemented in polynomial-time unless {\tt RP} $\supseteq$ {\tt NP}. 

\begin{theorem} \label{thm:hardness of unit-demand learning}
Suppose that a unit-demand\footnote{A {\em unit-demand} valuation $v$ is one satisfying $v(S)=\max_{i \in S} v(\{i\})$, for all $S \subseteq [m]$.} bidder whose value for each item $i\in [m]$ is $v$ participates in a sequence of $T$ SiSPAs. Unless {\tt RP} $\supseteq$ {\tt NP}, there is no learning algorithm running in time polynomial in $m$, $v$, and $T$ and whose regret is any polynomial in $m$, $v$, and $1/T$. The computational hardness holds even when the learner faces i.i.d. samples from a fixed distribution of competing bids, and whether or not no-overbidding is required of the bids produced by the learner.
\end{theorem}

Note that our theorem proves an intractability result, even if pseudo-polynomial dependence on the description of $v$ is permitted in the regret bound and the running time. The {\em no-overbidding assumption} mentioned in the statement of our theorem represents a collection of conditions under which no-regret learning in second-price auctions gives good welfare guarantees~\cite{Christodoulou2008,Feldman2013}. An example of such no-overbidding condition is this: For each subset $S \subseteq [m]$, the sum of bids across items in $S$ does not exceed the bidder's value for bundle $S$. Sometimes this condition is only required to hold on average. It will be clear that our hardness easily applies whether or not no-overbidding is imposed on the learner, so we do not dwell on this issue more in this paper. The proof of Theorem~\ref{thm:hardness of unit-demand learning} is given in Section~\ref{sec:no regret hardness}, and obtained via two sub-results of interest:
\begin{itemize} %\medskip \noindent $\bullet$  
\item First, we show that it is {\tt NP}-hard to compute one step of the Follow-The-Leader (FTL) algorithm in SiSPAs, even for unit-demand bidders with the same value for all items, and even when this value is given in unary representation.  One way to view the problem that FTL faces in each step is this: Suppose that you are bidding against a single bidder, and you are given an explicit description of the distribution of his bid vector---that is, a list of bid vectors and their corresponding probabilities. What is the optimal vector of bids that you should place in the different auctions? It is easy to see that computing the optimal bid vector  is tantamount to computing one step of FTL. We show the following:

\begin{theorem}[Corollary of Theorem~\ref{thm:approx-optimal}] \label{thm:one step of FTL is hard} Computing one step of FTL in SiSPAs is {\tt NP}-hard, even for a unit-demand bidder whose values for all items are the same and are given in unary. In fact, %the problem facing FTL in the $t$-th step 
it is {\tt NP}-hard to approximate to within an additive $1/2t$.
\end{theorem}
%Theorem~\ref{thm:one step of FTL is hard} is obtained by reducing from set cover.

%\medskip \noindent $\bullet$ 
\item We then use our inapproximability result for FTL, i.e. Theorem~\ref{thm:one step of FTL is hard}, to get our impossibility result for any polynomial-time no-regret learning algorithm, i.e. Theorem~\ref{thm:hardness of unit-demand learning}. We show that this is a general phenomenon: whenever one step of FTL is inapproximable, there is no polynomial-time no-regret learning algorithm. 
\begin{theorem} \label{thm:LB for FTL implies general LB}
Consider a family  ${\cal F}$ of functions $f:{\cal X} \rightarrow [0,v]$, and suppose that $b$ bits suffice to index each function in $\cal F$ and element in $\cal X$ under some encoding. Suppose also that, given an explicit description of a distribution ${\cal D}$ over ${\cal F}$\footnote{The size of the description is the total number of bits needed to index the functions in its support and the probabilities assigned to them.} as well as $v$ in unary representation, it is {\tt NP}-hard to find some $x \in {\cal X}$ whose expected value $\E_{f \sim D}[f(x)]$ is within an additive $O(1/|D|^c)$ of the optimum for some constant $c>0$, where $|D|$ is the size of $D$'s support. Then, unless {\tt RP} $\supseteq$ {\tt NP}, there is no learning algorithm running in time polynomial in $b$, $v$, and $T$ and whose regret after $T$ steps is any polynomial in $b$, $v$, and $1/T$.
\end{theorem}
Observe that the hypothesis of Theorem~\ref{thm:LB for FTL implies general LB} is tantamount to the problem facing FTL in a learning environment with cost functions ${\cal F}$. Our statement is also careful to cater for pseudo-polynomial dependence of the regret bound on the diameter $v$ of the range of our cost functions, as the typical dependence of no-regret learning algorithms on the diameter is pseudo-polynomial, and we are seeking to get lower bounds for such learners.
\end{itemize}

Our intractability results cast shadow in the ability of computationally bounded learners to achieve no-regret guarantees, thereby converging to approximately efficient outcomes in SiSPAs. We remedy this state of affairs by proposing a new type of learning dynamics that we call ``no-envy,'' which are both efficiently computable, and achieve strong welfare guarantees, as we argue below.

\paragraph{No-Envy Dynamics: Computation and Welfare.} No-envy dynamics are a twist to no-regret dynamics. Recall that in no-regret dynamics the requirement is that the cumulative utility of the bidder after $T$ rounds be within an additive $o(T)$ of the optimum utility he could have achieved in hind-sight through the best fixed bid vector. In no-envy dynamics, we require that the bidder's cumulative utility be within an additive $o(T)$ of the optimum utility that he would have achieved if he won the best in hind-sight bundle of items across all rounds, paying the running price of that bundle in each round. The guarantee is inspired by Walrasian equilibrium: In SiSPAs, the price that a bidder faces on each item is determined by the bids of the other players. Viewed as a price-taker, the bidder would want to achieve utility at least as large as the one he would have achieved if he purchased his favorite bundle at the prevailing prices. No-envy dynamics require that the average utility of the bidder across $T$ rounds is within $o(1)$ of what he would have achieved by purchasing the optimal bundle at the average price of each item across $T$ rounds. Besides providing a  natural regret guarantee, we show that no-envy dynamics are both efficiently computable, and result in efficient outcomes.

\paragraph{Efficient No-Envy Learning.} We show that no-envy learning can be efficiently attained for bidders with fractionally subadditive (XOS) valuations. A valuation $v(\cdot)$  belongs to this family if for some collection of vectors ${\cal V}=(v^\ell)_\ell \in \mathbb{R}_+^m$, it satisfies:
\begin{align} \label{eqn:XOS}
v(S)=\max_{\ell \in {\cal V}}\sum_{j \in S}v^{\ell}_j, \forall S \subseteq [m].
\end{align}
Note that XOS is a larger class than submodular valuations. In particular, given that the ${\cal V}$ describing an XOS valuation may be large, instead of inputting these valuations explicitly into our algorithms, we will assume that we are given an oracle, which given $S$ returns the vector $v^\ell \in {\cal V}$ such that $v(S) =  \sum_{j \in S}v^{\ell}_j$. We will call such an oracle an {\em XOS oracle}. We also sometimes assume, as it is customary in Walrasian equilibrium, that we are given access to a {\em demand oracle}, which given a price vector $p \in \mathbb{R}_+^m$ returns the bundle $S$ maximizing $v(S)-\sum_{j\in S}p_j$. We show the following.

\begin{theorem}\label{thm:XOS-demand}
Consider a bidder with an XOS valuation $v(\cdot)$ participating in a sequence of SiSPAs. Assuming access to a demand and an XOS oracle for $v(\cdot)$,\footnote{For submodular valuations this is equivalent to assuming access only to demand oracles, as XOS oracles can be simulated in polynomial time assuming demand oracles \cite{Dobzinski2010}} there exists a polynomial-time computable learning algorithm for computing the bidder's bid vector $b^t$ at every time step $t$ such that after $T$ iterations the bidder's average utility satisfies:
\begin{equation}
\frac{1}{T}\E\left[\sum_{t=1}^{T} u(b^t)\right] \geq \max_{S} \left(v(S) - \sum_{j\in S} \hat{\theta}_j^T\right)-\vsedit{O\left(\frac{m^2(D+H)}{\sqrt{T}}\right)},
\end{equation}
where $\hat{\theta}_j^T$ is the average cost of item $j$ in the first $T$ rounds of the dynamics as defined by the bids of the competing bidders, $D$ is a bound on the {competing bid} for any item and $H$ is an upper bound on $\max_S v(S)$. The learning algorithm with the above guarantee also satisfies the no overbidding condition that the sum of bids for any set of items is never larger than the bidder's value for that set. Moreover, the guarantee holds with no assumption about the behavior of competing bidders.
\end{theorem}

The proof of Theorem~\ref{thm:XOS-demand} is carried out in three steps, of which the first and last are specific to SiSPAs, while the second provides a general-purpose Follow-The-Perturbed-Leader (FTPL) algorithm in online learning scenarios where the number of experts is exponentially large and the {cost/utility} functions are arbitrary:
\begin{itemize}
\item The first ingredient is simple, using the XOS oracle to reduce no-envy learning in SiSPAs to no-regret learning in a related ``online buyer's problem,'' where the learner's actions are not bid vectors but instead what bundle to purchase, prior to seeing the prices; see Definition~\ref{def:online buyer's prob}. Theorem~\ref{lem:from sets to bids} provides the reduction from no-envy learning to this problem using XOS oracles. 

\item The second step proposes a FTPL algorithm for online learning problems where the learner chooses some action $a^t \in A$ and the environment chooses some state $\theta^t \in \Theta$, from possibly infinite, unstructured sets $A, \Theta$, while the learner's reward is tied to these choices through some function $u(a^t,\theta^t)$ that need not be linear. Since $A$ need not have finite-dimensional structure and $u$ need not be linear, we cannot efficiently simulate a perturbation of the cumulative reward of each element in $A$ to apply as in~\cite{Kalai2005}; see~\cite{Bubeck2012} and its references for an overview of such approaches. Instead of perturbing the cumulative rewards directly, our proposal is to do this indirectly by augmenting the history $\theta^1,\ldots,\theta^{t-1}$ that the learner has experienced so far with some randomly chosen fake history, and run FTL subject to these augmentations. While it is not a priori clear whether our perturbation approach is a useful one, it is clear that our proposed algorithm only needs an offline optimization oracle to be implemented. In Theorem~\ref{thm:general-regret}, we bound the regret experienced by our algorithm in terms of $u$'s stability. Roughly speaking, we want that our randomized augmentations smear the output of the offline optimization algorithm over $A$, allowing us to couple the choices of Be-The-Perturbed-Leader and Follow-The-Pertubed-Leader.

\item  The third step in our proof of Theorem~\ref{thm:XOS-demand} is to analyze the stability of the bidder's utility function in SiSPAs subject to the right choice of a history augmentation sampler. This is done in Section~\ref{sec:demand}. There turns out to be a simple sampler for our application here, where only one price vector is added to the history, whose prices are independently distributed according to an exponential distribution with mean $O(\sqrt{T})$ and variance $O(T)$.
\item While our motivation comes from mechanism design, our FTPL algorithm is general, and we believe will find applications in other settings. We provide some discussion in Section~\ref{sec:finite-parameter}, where we show how our algorithm implies regret bounds independent of $|A|$ when $\Theta$ is finite, as well as quantitative improvements on the regret bounds of~\cite{Balcan2015} for security games. %We also provide in Section~\ref{sec:contextual-bandits} an application of our general algorithm to the adversarial contextual experts problem, providing the first oracle-based algorithm for the adversarial setting.
\end{itemize}


%{\em capacitated fractionally sub-additive (C-XOS) valuations}, as long as the capacity is \vsedit{$O(\log(m))$. %an absolute constant. 
%A valuation function $v(\cdot)$ belongs to this family if, for some  $k =O(\log(m))$}, and a collection of $k$-sparse vectors $(v^\ell)_\ell \in \mathbb{R}_+^m$, it satisfies:
%$$v(S)=\max_{\ell}\sum_{j \in S}v^{\ell}_j, \forall S \subseteq [m].$$
%Clearly unit-demand valuations belong to this class with $k=1$. We show the following.
%
%\vscomment{Costi: DELETE the C-XOS and replace them with the XOS with demand oracles result. I will not refer to the Theorem 4 in the main text.}
%
%
%
%We show that no-envy learning can easily be attained for bidders with {\em capacitated fractionally sub-additive (C-XOS) valuations}, as long as the capacity is \vsedit{$O(\log(m))$. %an absolute constant. 
%A valuation function $v(\cdot)$ belongs to this family if, for some  $k =O(\log(m))$}, and a collection of $k$-sparse vectors $(v^\ell)_\ell \in \mathbb{R}_+^m$, it satisfies:
%$$v(S)=\max_{\ell}\sum_{j \in S}v^{\ell}_j, \forall S \subseteq [m].$$
%Clearly unit-demand valuations belong to this class with $k=1$. We show the following.
%\begin{theorem}\label{thm:XOS no envy}
%Consider a bidder with a C-XOS valuation $v(\cdot)$ participating in a sequence of SiSPAs. There exists a polynomial-time computable learning algorithm for computing the bidder's bid vector $b^t$ at every time step $t$ such that after $T$ iterations the bidder's average utility satisfies:
%\begin{equation}
%\frac{1}{T}\sum_{t=1}^{T} u(b^t) \geq \max_{S} \left(v(S) - \Theta^T(S)\right) - \max_S{v(S)}\sqrt{\frac{m}{T}},
%\end{equation}
%where $\Theta^T(S)$ is the average cost of set $S$ in the first $T$ rounds of the dynamics as defined by the bids of the competing bidders. The learning algorithm with the above guarantee also satisfies the no overbidding condition that the sum of bids for any set of items is never larger than the bidder's value for that set. Moreover, the guarantee holds with no assumption about the behavior of the competing bidders.
%\end{theorem}

%We also provide results 
In the absence of demand oracles, we provide positive results for the subclass of XOS called coverage valuations.
%two subclasses of XOS valuations: capacitated-XOS, and coverage valuations. Capacitated-XOS  are XOS valuations defined as in Eq~\eqref{eqn:XOS} by sets $\cal V$ that contain $k$-sparse vectors, for $k=O(\log m)$. (In particular these valuations contain unit-demand valuations.) In Section~\ref{sec:no-envy}, we observe that we can easily achieve no-regret learning in the online buyer's problem with capacitated-XOS valuations, and by Theorem~\ref{lem:from sets to bids} no-envy learning in SiSPAs. 
%With substantially more work, we can extend our no-envy dynamics to {\em coverage valuations}, albeit now our dynamics are approximately no-envy. 
To explain these valuations, consider a bidder with $k$ needs, $1,\ldots,k$, associated with values $a_1,\ldots,a_k$. There are $m$ available items, each covering a subset of these needs. So we can view each item as a set $\beta_i \subseteq [k]$ of the needs it satisfies. The value that the bidder derives from a set $S \subseteq [m]$ of the items is the total value from the needs that are covered, namely: $$v(S)=\sum_{\ell \in \cup_{j} \beta_j} a_\ell.$$
%We also provide results in the absense of demand oracles for two subclasses of XOS valuations: capacitated-XOS, and coverage valuations. Capacitated-XOS  are XOS valuations defined as in Eq~\eqref{eqn:XOS} by sets $\cal V$ that contain $k$-sparse vectors, for $k=O(\log m)$. (In particular these valuations contain unit-demand valuations.) In Section~\ref{sec:no-envy}, we observe that we can easily achieve no-regret learning in the online buyer's problem with capacitated-XOS valuations, and by Theorem~\ref{lem:from sets to bids} no-envy learning in SiSPAs. With substantially more work, we can extend our no-envy dynamics to {\em coverage valuations}, albeit now our dynamics are approximately no-envy. To explain these valuations, consider a bidder with $k$ needs, $1,\ldots,k$, associated with values $a_1,\ldots,a_k$. There are $m$ available items, each covering a subset of these needs. So we can view each item as a set $\beta_i \subseteq [k]$ of the needs it satisfies. The value that the bidder derives from a set $S \subseteq [m]$ of the items is the total value from the needs that are covered, namely:
%$$v(S)=\sum_{\ell \in \cup_{j} \beta_j} a_\ell.$$

%Our guarantees for coverage valuations are as follows:
\begin{theorem}\label{thm:main-coverage}
Consider a bidder with an explicitly given coverage valuation $v(\cdot)$ participating in a sequence of SiSPAs. There exists a polynomial-time computable learning algorithm for computing the bidder's bid vector $b^t$ at every time step $t$ such that after $T$ iterations the %average 
bidder's utility satisfies:
\begin{equation}
\frac{1}{T}\E\left[\sum_{t=1}^{T} u(b^t)\right] \geq \max_{S} \left(\left(1-\frac{1}{e}\right)v(S) - \sum_{j\in S} \hat{\theta}_j^T\right) - 3m\frac{H+\sqrt{D}}{\sqrt{T}},
\end{equation}
where $\hat{\theta}_j^T$, $H$ and $D$ are as in Theorem~\ref{thm:XOS-demand}, and the algorithm satisfies the same no overbidding condition stated in that theorem. There is no assumption about the behavior of the competing bidders.
%
%the average cost of set $S$ in the first $T$ rounds of the dynamics as defined by the bids of the competing bidders. The learning algorithm with the above guarantee also satisfies the no overbidding condition that the sum of bids for any set of items is never larger than the bidder's value for that set. Moreover, the guarantee holds with no assumption about the behavior of the competing bidders.
\end{theorem}
We prove Theorem~\ref{thm:main-coverage} via an interesting connection between the online buyer's problem for coverage valuations and the convex rounding approach for truthful welfare maximization proposed by~\cite{Dughmi2011}. In the online buyer's problem, recall that the buyer needs to decide what set to buy at each step, prior to seeing the prices. It is natural to have the buyer include each item to his set independently, thereby defining an expert for all points $x\in [0,1]^m$, where $x_i$ is the probability that item $i$ is included. It turns out that the expected utility of the buyer under such distribution $x$ is not necessarily convex, so this choice of experts turns our online learning problem non-convex. Instead we propose to massage each expert $x \in [0,1]^m$ into a distribution $D(x) \in \Delta(2^{[m]})$ and run online learning on the massaged experts. In Definition~\ref{def:convex rounding} we put forth conditions for the massaging operation $D(\cdot)$ under which online learning becomes convex and gives approximate no-regret (Lemma~\ref{lem:online-convex}). We then instantiate $D(\cdot)$ with the Poisson sampling of~\cite{Dughmi2011}, establishing Theorem~\ref{thm:main-coverage}. Our approach is summarized in Section~\ref{sec:convex} and the details can be found in Appendix~\ref{sec:app-convex}.

\paragraph{Welfare Maximization.}  Arguably one of the holy grails in Algorithmic Mechanism Design, since its inception, has been to obtain polynomial-time mechanisms optimizing welfare in incomplete information settings. Computational considerations aside, the VCG mechanism  optimizes welfare in all settings, and the challenge has been to determine whether computational boundedness of either the auctioneer or the bidders makes the task impossible. Much of the focus has been on combinatorial auction settings where $m$ items are sold to $n$ bidders, whose valuations $v_i(\cdot)$ are private information. In this setting, there exist poly-time computable dominant-strategy incentive compatible mechanisms that approximately optimize welfare when the bidders have coverage valuations. However, already for bidders with submodular valuations, there are quite severe inapproximability results~\cite{Dobzinski2011,Dughmi2015}. 

The literature on PoA of auctions alleviates this intractability by offering simple auctions, such as SiSPAs, where no-regret learning converges to outcomes whose welfare is approximately optimal. Except, our intractability results show that, in this case, bidders may be unable to run poly-time no-regret algorithms, even when they are unit-demand. At least, this is the case in SiSPAs.

We show that, if one is willing to accept no-envy learning as a solution concept, welfare can be approximately optimized all the way up to XOS valuations. In particular, we show that when bidders run no-envy or approximately no-envy dynamics, the welfare guarantees proven via PoA analysis can be recovered, with the added benefit that now bidders can be assumed polynomial-time bounded.

\begin{corollary} \label{cor:welfare guarantees}
When each bidder $i \in \{1,\ldots,n\}$ participating in a sequence of SiSPAs has an XOS valuation (endowed with a demand and XOS oracle) or an explicitly given coverage valuation $v_i(\cdot)$, there exists a polynomial-time computable learning algorithm such that, if each bidder $i$ employs this algorithm to compute his bids $b_i^t$ at each step $t$, then after $T$ rounds the average welfare is guaranteed to be at least:
\begin{equation}
\frac{1}{T}\E\left[\sum_{t=1}^{T} SW(b_1^t,\ldots,b_n^t)\right] \geq \frac{1}{2} \left(1-\frac{1}{e}\right)\opt(v_1,\ldots,v_n) -O\left( \vsedit{m^2}\cdot \vsedit{n \cdot} \max_{S,i}v_i(S) \sqrt{\frac{1}{T}}\right).
\end{equation}
If all bidders have XOS valuations with demand and XOS oracles the factor in front of OPT is $1/2$.
\end{corollary}

We view Corollary~\ref{cor:welfare guarantees}, in particular our result for XOS valuations with demand queries, as going a long way to alleviate the afore-described intractability results for submodular valuations. We provide what believe is a new perspective to mechanism design, namely mechanism design with no-envy bidders, obtaining positive results for the broader class of XOS valuations. In doing so, we provide an answer raised in~\cite{Feldman2015} about whether demand oracles can be exploited for welfare maximization with submodular bidders. We show a positive answer for the bigger class of XOS valuations, albeit with a different solution concept. (It still remains open whether there exist poly-time DSIC mechanisms for submodular bidders with demand queries.) We believe that no-envy learning is a fruitful new approach to mechanism design, discussing in Section~\ref{sec:general no envy definition} the meaning of the solution concept outside of SiSPAs.

\vsdelete{\paragraph{Related Work.} We have already placed our results in the context of the literature on no-regret learning, Price of Anarchy analysis of simple mechanisms, and Mechanism Design. The computational complexity of no-regret learning in simple mechanisms has been previously studied by Cai and Papadimitriou~\cite{Cai2014}, where it has been shown intractable, albeit in Bayesian settings, where hardness stems primarily from the distributions of player values. More recently, Hazan and Kozen~\cite{Hazan2015} have provided query complexity lower bounds for no-regret learning, when the learner only accesses his reward function via an optimization oracle. These query complexity lower bounds do not apply to the structured learning environments defined by SiSPAs. Due to space constraints more discussion of related work is given in Appendix~\ref{sec:app-related}.}

%\vscomment{This text was in the hardness section but should go somewhere in the intro or replaced by something similar in the intro: If we were in a complete information setting then we know by the results of Christodoulou et al. \cite{Christodoulou2008} that a pure Nash equilibrium of the complete information setting is computable in polynomial time. Hence, a trivial "no-regret" algorithm without the incomplete information condition is: each player computes the pure Nash equilibrium with the algorithm in \cite{Christodoulou2008} and submits the bid vector that corresponds to the outcome of these dynamics.}

%\vscomment{Costi mention something about general mechanisms and no-envy and taxation principle.}
%
%\vscomment{\paragraph{Related Work.} Cai and Papadimitriou. Markets for indivisible goods and relation to PoA?
%}

==> introduction.tex <==

Suppose that your boss assigned you the task of procuring items for your company. There are $m$ different items that you may procure, and your company's value for each bundle $S \subseteq [m]$ is specified by a valuation $v: 2^{[m]} \longrightarrow \mathbb{R}$. In fact, suppose that you need to do a fresh procurement every day for $T$ days. Making your task challenging is the fact that, each day, every item is sold separately through a second price auction, and these auctions are run in parallel. So, each day, you are called to place a bid in each single-item auction, and cannot express more complex preferences over bundles of items. Moreover, you have no information about who else may be participating in the various auctions or what their valuations might be, so you cannot predict the prices at which different items will end up selling each day.

Given your lack of information about the competition and your inability to express complex preferences, a natural guarantee you may want to achieve is {\em no-regret}: that your cumulative utility over $T$ procurements is within an additive $o(T)$ of the cumulative utility that you would have achieved in hindsight from the best vector of bids $b_1,\ldots,b_m$, if you were to place the same bid $b_i$ in the second-price auction for item $i$ across all $T$ periods. 

Besides being motivated from an online learning point of view, a growing volume of recent papers has shown that no-regret learning in auction environments also achieves surprising welfare guarantees~\cite{Bikhchandani99,??}. For example, when bidders whose valuations are subadditive\footnote{A {\em subadditive} valuation $v$ is one satisfying $v(S \cup T) \le v(S)+v(T),$ for all $S, T \subseteq [m]$.} use no-regret learning to choose their bids in repeated simultaneous second-price auctions, the average welfare converges to a quarter of that achieved by the optimal allocation~\cite{FeldmanFGL13}. Similar guarantees hold for simultaneous first-price auctions or other types of compositions of simple auctions~\cite{SyrkanisT}. This guarantee is astounding, given the impossibility results for dominant solvable mechanisms, even for submodular\footnote{A {\em submodular} valuation $v$ is one satisfying $v(S\cup T) + v(S \cap T) \le v(S)+v(T)$, for all $S, T \subseteq [m]$.} bidders~\cite{??}. 

The robustness of no-regret learning with respect to players' information and its strong welfare guarantees motivates us to study its computational complexity. We show that in one of the most basic settings where no-regret learning is non-trivial, it cannot be implemented in polynomial-time unless {\tt RP} $\supseteq$ {\tt NP}. 

\begin{theorem} \label{thm:hardness of unit-demand learning}
Suppose that a unit-demand\footnote{A {\em unit-demand} valuation $v$ is one satisfying $v(S)=\max_{i \in S} v(\{i\})$, for all $S \subseteq [m]$.} bidder whose value for each item $i\in [m]$ is $v$ participates in a sequence of $T$ simultaneous second-price auctions. Unless {\tt RP} $\supseteq$ {\tt NP}, there is no learning algorithm running in time polynomial in $m$, $v$, and $T$ and whose regret is any polynomial in $m$, $v$, and $1/T$. The computational hardness holds even when the learner faces i.i.d. samples from a fixed distribution of competing bids, and whether or not no-overbidding is required of the bids produced by the learner.
\end{theorem}

Note that our theorem proves an intractability result, even if pseudo-polynomial dependence on the description of $v$ is permitted in the regret bound and the running time. The {\em no-overbidding assumption} mentioned in the statement of our theorem represents a collection of conditions under which no-regret learning in second-price auctions gives good welfare guarantees~\cite{FeldmanFGL13,...}. An example of such no-overbidding condition is this: For each subset $S \subseteq [m]$, the sum of bids across items in $S$ does not exceed the bidder's value for bundle $S$. Sometimes this condition is only required to hold on average. It will be clear that our hardness easily applies whether or not no-overbidding is imposed on the learner, so we do not dwell on this issue more in this paper. The proof of Theorem~\ref{thm:hardness of unit-demand learning} is given in Section~\ref{sec:no regret hardness}, and obtained via two sub-results of interest:
\begin{itemize}
\item In Section~\ref{sec:inapproximability of best response}, we show that it is {\tt NP}-hard to compute one step of the Follow-The-Leader (FTL) algorithm in simultaneous second price auctions, even for unit-demand bidders with the same value for all items, and even when this value is given in unary representation.  One way to view the problem that FTL faces in each step is this: Suppose that you are bidding against a single bidder, and you are given an explicit description of the distribution of his bid vector---that is, a list of bid vectors and their corresponding probabilities. What is the optimal vector of bids that you should place in the different auctions? It is easy to see that computing the optimal bid vector  is tantamount to computing one step of FTL. We show the following:
\begin{theorem}[Corollary of Theorems~\ref{thm:exact-optimal} and~\ref{thm:approx-optimal}] \label{thm:one step of FTL is hard} Computing one step of FTL in simultaneous second-price auctions is {\tt NP}-hard, even for a unit-demand bidder whose values for all items are the same and are given in unary. In fact, the problem facing FTL in the $t$-th step is {\tt NP}-hard to approximate to within an additive $1/2t$.
\end{theorem}
%Theorem~\ref{thm:one step of FTL is hard} is obtained by reducing from set cover.
\item In Section~\ref{sec:from inapproximability of best response to NP-hardness of no-regret}, we use our inapproximability result for FTL, i.e. Theorem~\ref{thm:one step of FTL is hard}, to get our impossibility result for any polynomial-time no-regret learning algorithm, i.e. Theorem~\ref{thm:hardness of unit-demand learning}. We show that this is a general phenomenon: whenever one step of FTL is inapproximable, there is no polynomial-time no-regret learning algorithm.
\begin{theorem} \label{thm:LB for FTL implies general LB}
Consider a family  ${\cal F}$ of functions $f:{\cal X} \rightarrow [0,v]$, and suppose that $b$ bits suffice to index each function in $\cal F$ and element in $\cal X$ under some encoding. Suppose also that, given an explicit description of a distribution ${\cal D}$ over ${\cal F}$\footnote{The size of the description is the total number of bits needed to index the functions in its support and the probabilities assigned to them.} as well as $v$ in unary representation, it is {\tt NP}-hard to find some $x \in {\cal X}$ whose expected value $\E_{f \sim D}[f(x)]$ is within an additive $O(1/|D|^c)$ of the optimum for some constant $c>0$, where $|D|$ is the size of $D$'s support. Then, unless {\tt RP} $\supseteq$ {\tt NP}, there is no learning algorithm running in time polynomial in $b$, $v$, and $T$ and whose regret after $T$ steps is any polynomial in $b$, $v$, and $1/T$.
\end{theorem}
Observe that the hypothesis of Theorem~\ref{thm:LB for FTL implies general LB} is tantamount to the problem facing FTL in a learning environment with cost functions ${\cal F}$. Our statement is also careful to cater for pseudo-polynomial dependence of the regret bound on the diameter $v$ of the range of our cost functions, as the typical dependence of no-regret learning algorithms on the diameter is pseudo-polynomial, and we are seeking to get lower bounds for such learners.
\end{itemize}

Our intractability result 


\paragraph{Related Work.} Cai and Papadimitriou. Markets for indivisible goods and relation to PoA?



==> low-dimensional.tex <==

In this section we consider the setting, where the sufficient statistics for computing the offline best action, lie in a $d$-dimensional space. We consider the general online learning problem, where the player picks an action $a\in A$, the adversary picks a parameter $\theta\in \Theta$ and the reward is $u(a,\theta)$. We will assume that $u(a,\theta)\in [-f_-(\theta),f_+(\theta)]$.

\paragraph{Low-dimensional sufficient statistics.} We will assume that for any $\theta^{1:T}$, there exists a mapping $\phi(\theta^{1:T}) \in \R^d$, such that:
\begin{equation}
M(\theta^{1:T}) = M\left(\phi\left(\theta^{1:T}\right)\right)
\end{equation}
We will refer to $\phi(\theta^{1:T})$ as the \emph{sufficient statistics} of sequence $\theta^{1:T}$.
We will assume that the sufficient statistics are \emph{linear}, in the sense that for any two sequences $\{x\}$ and $\{y\}$: 
\begin{equation}
\phi(\{x\}\cup\{y\}) = \phi(\{x\})+\phi(\{y\})
\end{equation}
Last we also assume that the difference in the sufficient statistics between two sequences that have length difference of $1$, is uniformly bounded by  some function of the extra parameter sample, i.e. for any sequence $\{x\}$ and for any parameter $\theta$:
\begin{equation}
\forall \{x\}: \|\phi(\{x\}\cup \theta)- \phi(\{x\})\|_1 \leq q(\theta)
\end{equation}
with respect to some norm $\|\cdot\|$.

\paragraph{Exponential inducing sample perturbation.} We also need that there exists a distribution over sequences $\{x\}$, such that the induced distribution over $\phi(\{x\})$ follows an independent symmetric exponential distribution on each coordinate, with parameter $\epsilon$, i.e. the density of the random variable $\phi(\{x\})$ at some point $k$ is $f(k) \propto \exp\{-\epsilon\|k\|_1\}$. We will denote the distribution over sample sequences $\{x\}$, which induces the latter exponential sufficient statistic distribution as the \emph{exponential inducing sample perturbation}.

We show that Algorithm \ref{defn:lazy-ftpl} with an exponential inducing sample perturbation is \emph{stable}.

\begin{lemma}[Stability lemma]\label{lem:statistic-stability} For any sequence $\theta^{1:T}$, such that $q(\theta^t)\leq D$ for all $t\in [T]$, the stability of Algorithm~\ref{defn:lazy-ftpl} with an exponential inducing sample perturbation is upper bounded by:
\begin{equation}
\E_{x}\left[u(M(\{x\}\cup \theta^{1:t}),\theta^t)-u( M(\{x\}\cup \theta^{1:{t-1}}), \theta^t)\right]\leq  \epsilon\cdot D \cdot f_+(\theta^t)
\end{equation}
\end{lemma}


Applying Theorem \ref{thm:general-regret}, we get:
\begin{theorem}\label{thm:statistic-regret}
For any sequence $\theta^{1:T}$, such that $q(\theta^t)\leq D$ for all $t\in [T]$, the regret of Algorithm~\ref{defn:lazy-ftpl} with an exponential inducing sample perturbation $\{x\}$, against oblivious adversaries is upper bounded by:
\begin{equation}
\sup_{a^*\in A}\E_{\{x\}}\left[\sum_{t=1}^T \left( u(a^*,\theta^t) - u(a^t,\theta^t)\right)\right] \leq \epsilon\cdot D\cdot \sum_{t=1}^T f_+(\theta^t) +  \E_{\{x\}}\left[\sum_{x^{\tau}\in \{x\}} \left(f_-(x^\tau)+f_+(x^\tau)\right)\right]
\end{equation}
Hence, the regret of Algorithm~\ref{defn:ftpl} against adaptive adversaries is bounded by the same amount. 
\end{theorem}






==> no-envy-set.tex <==
%
%  Created by WinFIG version 6.0 final 
%  METADATA <version>1.0</version> 
%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5510,2534)(1643,-1978)
%  METADATA <id>2</id> 
{\color[rgb]{0,0,0}\thinlines
\put(2602,-695){\oval(1440,1186)}
}%
%  METADATA <id>3</id> 
{\color[rgb]{0,0,0}\put(3032,-702){\oval(2468,1652)}
}%
%  METADATA <id>4</id> 
{\color[rgb]{0,0,0}\put(3912,-692){\oval(4366,2138)}
}%
%  METADATA <id>5</id> 
{\color[rgb]{0,0,0}\put(4398,-711){\oval(5494,2518)}
}%
%  METADATA <id>9</id> 
\put(4292,-497){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}CCE $\equiv$ No-Regret}%
}}}}
%  METADATA <id>10</id> 
\put(6197,-497){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}No-Envy}%
}}}}
%  METADATA <id>13</id> 
\put(2450,-497){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}NE}%
}}}}
%  METADATA <id>15</id> 
\put(4628,-778){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}PoA $\leq 2$}%
}}}}
%  METADATA <id>16</id> 
\put(4564,-1092){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Intractable}%
}}}}
%  METADATA <id>17</id> 
\put(6216,-778){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}PoA $\leq 2$}%
}}}}
%  METADATA <id>18</id> 
\put(6185,-1092){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Tractable}%
}}}}
%  METADATA <id>22</id> 
\put(2229,-778){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}PoA $\geq 2$}%
}}}}
%  METADATA <id>14</id> 
\put(3545,-497){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}CE}%
}}}}
\end{picture}%


==> oracle.tex <==
In this section we examine whether we can actually achieve the stronger no-regret property, rather than the no-envy property, in the online bidding problem against adversaries, assuming that we are given an offline bidding optimization oracle. We give a brief exposition of our results here and defer the full analysis to Appendix~\ref{sec:app-finite}

We show that if the adversary can pick one among $d$ possible threshold vectors on each day, then there exists an efficient no-regret algorithm for the online bidding problem against adversaries, assuming that we have oracle access to the offline optimization problem. Observe that this problem is highly non-trivial, as without the optimization oracle, our impossibility result covers such settings, since in the set cover reduction, the number of different price vectors used was at most $r\cdot m$, which is finite and polynomial in the description of the instance. Yet, without an oracle there does not exist any polynomial time no-regret algorithm. We will show that in such settings an optimization oracle bypasses this impossibility. 

\paragraph{General online learning with finite parameter space.} We  actually show this for the general online learning problem which we defined in the beginning of this section, which could be of independent interest and which nicely complements recent impossibility results of \cite{Hazan2015}. Specifically, we show that in any online learning problem where the adversary has only $d$ choices to pick from on each day, i.e. $|\Theta|=d$, then with an access to an offline optimization problem an instantiation of Algorithm~\ref{defn:lazy-ftpl}, can achieve regret of $2H\sqrt{d/T}$, assuming utilities are bounded in $[0,H]$. This regret is independent of the number of available actions! 

\paragraph{Security games.} Apart from the application to our online bidding problem, we show that this result finds interesting application in the security game model of \cite{Balcan2015}, yielding improved regret rates and computationally efficient algorithms assuming offline oracles (see Section~\ref{sec:app-security}). 




